Ray-of-Arrival Passing for Indirect Beam Training in Cooperative Millimeter Wave MIMO Networks

This paper is concerned with the channel estimation problem in multi-cell Millimeter (mmWave) wireless systems. We develop a novel Ray-of-Arrival Passing for Indirect (RAPID) Beam Training framework, in which a network consisting of multiple BS are able to work cooperatively to estimate jointly the UE channels. To achieve this aim, we consider the spatial geometry of the mmWave environment and transform conventional angular domain beamforming concepts into the more euclidean, Ray-based domain. Leveraging this model, we then consider the conditional probabilities that pilot signals are received in each direction, given that the deployment of each BS is known to the network. Simulation results show that RAPID is able to improve the average estimation of the network and significantly increase the rate of poorer quality links. Furthermore, we also show that, when a coverage rate threshold is considered, RAPID is able to improve greatly the probability that multiple link options will be available to a user at any given time.

==> Compiler-LaTeX/Arco-list.tex <==

\newacronym{mmWave}{mmWave}{millimeter wave}	

\newacronym{ADC}{ADC}{analog-to-digital converter}
\newacronym{DAC}{DAC}{digital-to-analog converter}
\newacronym{SNR}{SNR}{signal-to-noise ratio}

\newacronym{BS}{BS}{base station}
\newacronym[plural={UEs},longplural={user equipment}]{UE}{UE}{user equipment}


\newacronym{PEE}{PEE}{probability of estimation error}
\newacronym{MIMO}{MIMO}{multiple-input multiple-output}
\newacronym{ULA}{ULA}{uniform linear array}

\newacronym{LMMSE}{LMMSE}{linear minimum mean squared estimator}
\newacronym{ML}{ML}{maximum likelihood}
\newacronym{CS}{CS}{compressed sensing}

\newacronym{RDB}{RDB}{random directional beamforming}
\newacronym{ES}{ES}{exhaustive search}


\newacronym[plural={AODs},longplural={angles of departure}]{AOD}{AOD}{angle of departure}
\newacronym[plural={AOAs},longplural={angles of arrival}]{AOA}{AOA}{angle of arrival}


\newacronym[plural={RODs},longplural={rays of departure}]{ROD}{ROD}{ray of departure}
\newacronym[plural={ROAs},longplural={rays of arrival}]{ROA}{ROA}{ray of departure}

\newacronym{AFC}{AFC}{analog fountain code}

\newacronym{GAMP}{GAMP}{generalized approximate message passing}
\newacronym{LASSO}{LASSO}{least absolute shrinkage and selection operator}

\newacronym{BG}{BG}{Bernoulli Gaussian}    

\newacronym{FCE}{FCE}{fast channel estimation}    
\newacronym{SWIFT}{SWIFT}{simultaneous estimation with iterative fountain training}
\newacronym{RAPID}{RAPID}{ray-of-arrival passing for in-direct}
\newacronym{RACE}{RACE}{rate adaptive channel estimation}



==> Compiler-LaTeX/layout.tex <==
%!TEX root = ../Thesis.tex

%%================= Page Layout ======================%%
% Page Layout
\setlength{\topmargin}{0cm}
\setlength{\textheight}{624pt}
\setlength{\textwidth}{6in}
\raggedbottom

% use these for two sided (even on left)
\setlength{\oddsidemargin}{0.0in}
\setlength{\evensidemargin}{0.267in}
% use this for one sided printing with thick left margin
%\setlength{\oddsidemargin}{0.4in}

\setlength{\columnwidth}{\textwidth}
\setlength{\footskip}{0.3in}
\setlength{\headheight}{16pt}                       % todo --- apparently 15pt is the minimum (?)

% Paragraph Layout
%\setlength{\parindent}{0em}                         % paragraph indent --- I prefer a space between paragraphs to indents
\setlength{\parskip}{1.5ex plus0.5ex minus0.5ex}    % space after paragraph (rubber length)
\renewcommand{\baselinestretch}{1.55}                % line spacing

% Float Settings
% When using defaults, latex produces many pages with stand-alone figures.
% These settings are meant to improve this a bit; feel free to fiddle with 
% them depending on the sizes and quantity of floating environments you use
\renewcommand{\topfraction}{0.85}
\renewcommand{\bottomfraction}{0.85}
\renewcommand{\textfraction}{0.2}
\renewcommand{\floatpagefraction}{0.2}
\setcounter{topnumber}{2}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{4}

%%================= Misc Global Settings =============%%
% how far down section numbers go (chapter/section/subsection/subsubsection/paragraph...)
\setcounter{secnumdepth}{2}

% how far down the TOC goes (chapter/section/subsection/subsubsection...)
%\setcounter{tocdepth}{2}

% Allow pagebreaks in equations
% Currently set to 1 = "if they absolutely must" (see amsmath documentation for more info)
\allowdisplaybreaks[1]


